Consistency of orthology and paralogy constraints in the presence of gene transfers

Orthology and paralogy relations are often inferred by methods based on gene similarity, which usually yield a graph depicting the relationships between gene pairs. Such relation graphs are known to frequently contain errors, as they cannot be explained via a gene tree that both contains the depicted orthologs/paralogs, and that is consistent with a species tree $S$. This idea of detecting errors through inconsistency with a species tree has mostly been studied in the presence of speciation and duplication events only. In this work, we ask: could the given set of relations be consistent if we allow lateral gene transfers in the evolutionary model? We formalize this question and provide a variety of algorithmic results regarding the underlying problems. Namely, we show that deciding if a relation graph $R$ is consistent with a given species network $N$ is NP-hard, and that it is W[1]-hard under the parameter "minimum number of transfers". However, we present an FPT algorithm based on the degree of the $DS$-tree associated with $R$. We also study analogous problems in the case that the transfer highways on a species tree are unknown.

==> indepSetReduction.tex <==

THIS SECTION IS UNDER CONSTRUCTION

We show that the following problem is NP-hard: Given a (least-resolved) DS-tree $G_{DS}$ for $\Gamma$ and a species network $N$ for $\Sigma$, decide whether there exists a CDST-completion $G$ of $G_{DS}$ such that $G$ is consistent with $N$.

We give a reduction from the NP-hard problem {\sc Independent Set}: given a graph $H=(V,E)$ and an integer $k$, decide whether there exists a set $V' \subseteq V$ such that $|V'| \ge k$ and $\{u,v\} \setminus V' \neq \emptyset$ for any edge $uv \in E$. We call such a set $V'$ an \emph{independent set of size $k$}


The intuition behind our construction is as follows: for each vertex in $H$ there will be a node in our species network whose descendants have transfer arcs leading to nodes representing the edges with which that vertex is incident. Our DS-tree will require us to use at least one transfer arc to each edge node. Our choice of DS-tree will also force us to choose $k$ vertex nodes as the members of our independent set, but choosing a given vertex will 'block' the transfer nodes leading to edges from that vertex node.  Thus, each edge must be incident with at least one vertex not chosen. It follows that our choice of $k$ vertices must indeed form an independent set. 



Let $(H=(V,E), k)$  be an instance of {\sc Independent Set}. 
Let $v_1, v_2, \dots, v_n$ be a numbering of the vertices in $V$, and $e_1, e_2, \dots, e_m$ a numbering of the edges in $E$.
We construct an instance of [our problem] as follows.

[Note: I was fairly fussy about distinguishing between the *leaf* of a gene / species tree, and the gene/ species that leaf is labelled with. We may wish to change this.]



\begin{itemize}
 \item Let $\Sigma$ consist of a species $specVert_i$ for each vertex $v_i$, a species $specEdge_j$ for each edge $e_j$, and four special species $specLeft$, $specRight$, $specIn$, $specOut$. (Note that our DS-tree will not use any genes from $specVert_i$ for any vertex $v_i$, but we need them for the construction of our species network.)
 \item To describe our species network, we first describe the distinguished base tree after indegree-$1$ and outdegree-$1$ nodes have been contracted. Let $r$ be the root node, with children $x_0$ and $y_0$.
 
 Let $x_0$ have children $leafLeft$ and $x_1$.
%  , with the leaf $leafLeft$ labelled with $specLeft$.
 For $i \in [n-2]$, let $x_i$ have children $leafVert_i$ and $x_{i+1}$, and let $x_{n-1}$ have children $leafVert_{n-1}$ and $leafVert_n$.
%  Let each leaf node $leafVert_i$ be labelled with $specVert_i$.
 
 Let $y_0$ have children $y_1$ and $z_0$.
 For each $j \in [m-2]$, let $y_j$ have children $leafEdge_j$ and $y_{j+1}$, and let $y_{m-1}$ have children $leafEdge_{m-1}$ and $leafEdge_m$.
%  Let each leaf node $leafEdge_j$ be labelled with $specEdge_j$.
 
 Finally let $z_0$ have children $leafIn$ and $z_1$, and let $z_1$ have children $leafOut$ and $leafRight$.
%  Let the leaf nodes $leafIn, leafOut, leafRight$ be labelled with $specIn, specOut$ and $specRight$ respectively.
 
 
 [We label the leaf nodes with species as follows. 
 Leafs $leafLeft$, $leafRight$, $leafIn$ and $leafOut$ are labelled with species $specLeft$, $specRight$, $specIn$ and $specOut$ respectively.
 For each $i \in [n]$, let leaf node $leafVert_i$ be labelled with $specVert_i$, and for each $j \in [m]$, let $leafEdge_j$ be labelled with $specEdge_j$.]
 
 \item We now describe how to subdivide edges and add secondary arcs in order to get our species network $N$.
 The order in which we subdivide edges will be important for the purposes of preserving time-consistency.
 
 For each $i \in [n]$ in order, do the following: 
 Subdivide the arc between $leafVert_i$ and its parent with a new node $tailVert_iIn$, and subdivide the arc between $leafIn$ and its parent with a new node $headVert_iIn$. Add $(tailVert_iIn,headVert_iIn)$ as an arc in $E_s$.
 
 Then, for each $j \in [m]$ in order, such that vertex $v_i$ is incident with edge $e_j$, do the following: Subdivide the arc between $leafVert_i$ and its parent with a new node $tailVert_iEdge_j$, and subdivide the arc between $leafEdge_j$ and its parent with a new node $headVert_iEdge_j$. Add $(tailVert_iEdge_j, headVert_iEdge_j)$ as an arc in $E_s$.
 
 Finally, subdivide the arc between $leafVert_i$ and its parent with a new node $tailVert_iOut$, and subdivide the arc between $leafOut$ and its parent with a new node $headVert_iOut$. Add $(tailVert_iOut,headVert_iOut)$ as an arc in $E_s$.
 
 \item After this process is complete, add any arcs not in $E_s$ to $E_p$, and we have our  species network $N$. We show that $N$is time-consistent as follows: let $t: \{r,x_0, \dots, x_n, y_0, \dots, y_m, z_0, z_1\} \rightarrow \mathbb{N}$ be an arbitrary function such that $t(u) < t(v)$ whenever $u$ is an ancestor of $v$.
 Let $n_0$ be the maximum value assigned by $t$, and now extend $t$ as follows.  
 For each $i \in [n]$, let $t(tailVert_iIn) = t(headVert_iIn) = n_0 + i$.
 For each $i \in [n]$ and each $j \in [m]$ such that  vertex $v_i$ is incident with edge $e_j$, let  $t(tailVert_iEdge_j) = t(headVert_iEdge_j) = n_0 + n + m(i-1) + j$.
 For each $i \in [n]$, let $t(tailVert_iOut) = t(headVert_iOut) = n_0 + n + mn + i$.
 Finally, for each  leaf node $leaf$, let $t(leaf) = n_0 + n + mn + n + 1$.
 
 It is straightforward (hopefully) to verify that $t$ satisfies the requirements for time-consistency.
 
 (Note that so far, we have not used the parameter $k$ in our construction).
 
 \item 
 Let $\Gamma$ consist of a gene $geneEdge_j$ assigned to $specEdge_j$ for each $j \in [m]$, a gene $geneLeft$ assigned to $specLeft$, a gene $geneRight$ assigned to $specRight$, and for each $h \in [k]$, a gene $geneIn_h$ assigned to $specIn$ and a gene $geneOut_h$ assigned to $specOut$. 
 
 \item We now describe our (least-resolved) DS-tree $G_{DS}$.

 Let the root of $G_{DS}$ be a speciation node $spec_0$. 
 Let the children of $spec_0$ be a duplication node $dup_0$ and a leaf node $leafGeneRight$.
 Let the children of $dup_0$ be a leaf node $leafGeneLeft$ and a speciation node $spec_1$.
 
 Let the children of $spec_1$ consist of a leaf node $leafGeneEdge_j$ for each $j \in [m]$, and a duplication node $dup_h$ for each $i \in [k]$.
 
 For each $h \in [k]$, let the children of $dup_h$ be a leaf node $leafGeneIn_h$ and a leaf node $leafGeneOut_h$.
 
 
[We label the leaf nodes of $G$ with genes as follows.
 Leafs $leafGeneLeft$ and $leafGeneRight$ are labelled with $geneLeft$ and $geneRight$ respectively.
 For each $j \in [m]$, the leaf node $leafGeneEdge_j$ is labelled with $geneEdge_j$.
 For each $h\in [k]$, leafs $leafGeneIn_h$ and $leafGeneOut_h$ are labelled with $geneIn_h$ and $geneOut_h$ respectively.]
 
 This concludes the construction of $G_{DS}$, and of our [problem] instance.
 
 
\end{itemize}


\begin{figure}
   \tikzstyle{spec}=[circle, fill=black, minimum size=3pt]
  \tikzstyle{dup}=[square, fill=black,  minimum size=8pt]
  \tikzstyle{dupedge} = [edge from parent path=     {(\tikzparentnode.south) -- (0,\levdist)  -- (\tikzchildnode.north)}] 
  \tikzstyle{specedge} = [edge from parent path=     {(\tikzparentnode.south) --  (\tikzchildnode.north)}] 
 \begin{tikzpicture}
\tikzstyle{level 1}=[sibling distance=3cm]
\tikzstyle{level 2}=[sibling distance=3cm]
\tikzstyle{level 3}=[sibling distance=3cm]
\tikzstyle{level 4}=[sibling distance=2.5cm]
\foreach \levdist in {1.5cm}
% \foreach \dupchild in {edge from parent path=     {(\tikzparentnode.center) -- (0,\levdist)  -- (\tikzchildnode.north)}}
{
  \node [] {$spec_0$}
 [level distance = \levdist]
  child[specedge] {node [] {$dup_0$}
    child[specedge] {node [] {$leafGeneLeft$}}
    child[specedge] {node [] {$spec_1$}
      child[specedge] {node {$leafGeneEdge_1$...}}
      child[specedge] {node {...$leafGeneEdge_m$}}
      child[specedge] {node {$dup_1$...}
        child[specedge] {node {$leafGeneIn_1$}}
        child[specedge] {node {$leafGeneOut_1$}}
        }
      child[specedge] {node {...$dup_k$}}
    }
  }
    child[specedge] {node [] {$leafGeneRight$}};
}
% \caption{Heloooo}
\end{tikzpicture}
 \caption{The DS-tree $G_{DS}$.}
\end{figure}

 
 
 
 
 
 \begin{figure}
   \tikzstyle{spec}=[circle, fill=black, minimum size=3pt]
  \tikzstyle{dup}=[square, fill=black,  minimum size=8pt]
  \tikzstyle{dupedge} = [edge from parent path=     {(\tikzparentnode.south) -- (0,\levdist)  -- (\tikzchildnode.north)}] 
  \tikzstyle{specedge} = [edge from parent path=     {(\tikzparentnode.south) --  (\tikzchildnode.north)}] 
 \begin{tikzpicture}
\tikzstyle{level 1}=[sibling distance=8.5cm]
\tikzstyle{level 2}=[sibling distance=3.5cm]
\tikzstyle{level 3}=[sibling distance=2cm]
\tikzstyle{level 4}=[sibling distance=2cm]
\tikzstyle{level 5}=[sibling distance=2.5cm]
\foreach \levdist in {1.5cm}
% \foreach \dupchild in {edge from parent path=     {(\tikzparentnode.center) -- (0,\levdist)  -- (\tikzchildnode.north)}}
{
  \node [] {$r$}
 [level distance = \levdist]
  child[specedge] {node [] {$x_0$}
    child[specedge] {node [] {$leafLeft$}}
    child[specedge] {node [] {$x_1$}
      child[specedge] {node {$TailVert_1In$}
        child[] {node{$leafVert_1$}}
      }
      child[specedge] {node {...}
        child[specedge] {node {}}
        child[specedge] {node {$x_{n-1}$}
          child[specedge] {node {$TailVert_{n-1}In$}
            child[] {node{$leafVert_{n-1}$}}
          }
          child[specedge] {node {$TailVert_nIn$}
            child[] {node{$leafVert_n$}}
          }
        }
      }
    }
  }
  child[specedge] {node [] {$y_0$}
    child[specedge] {node [] {$y_1$}
      child[specedge] {node {$leafEdge_1$}}
      child[specedge] {node {...}
        child[specedge] {node {}}
        child[specedge] {node {$y_{m-1}$}
          child[specedge] {node {$leafEdge_{m-1}$}}
          child[specedge] {node {$leafEdge_m$}}
        }
      }
    }   
    child[specedge] {node [] {$z_0$}
      child[specedge] {node [] {$leafIn$}}
      child[specedge] {node [] {$z_1$}
        child[specedge] {node [] {$leafOut$}}
        child[specedge] {node [] {$leafRight$}}
      }
    }
  };
}
% \caption{Heloooo}
\end{tikzpicture}
 \caption{The network $N$. Transfer arcs and their vertices (except for $TailVert_iIn$) are not pictured.}
\end{figure}
 
\begin{lemma}
 Suppose that  there is a $CDST$-completion $G$ of $G_{DS}$ such that $G$ is consistent with $N$. Then $H$ has an independent set $V'$ of size $k$. 
\end{lemma}

\begin{proof}
 Recall that $G$ is derived from $G$ by refining non-binary nodes into binary subtrees (made of nodes of the same type), [subdiving edges], relablling some duplication or speciation nodes as transfer nodes, and marking at least one out-arc ofeach transfer node as a transfer arc.
 
 Let $s:V(G) \rightarrow V(N)$ be a consistent gene-mapping.
 
 We will speak of a subtree of $G$ as ``corresponding'' to a vertex in $G_{DS}$ when that subtree was the result of refining the vertex.
 Similarly we may speak of a single vertex in $G$ as corresponding to a vertex in $G_{DS}$ if that vertex was not refined.
 We note that the binary nodes in $G_{DS}$ (such as $dup_h$ for each $h \in [k]$) cannot be refined, and for such nodes $v$ there must be a single nodes in $G$ corresponding to $v$.
 In such cases we will refer to the node corresponding to $v$ by the name $v$ as well.
 We also note that every leaf in $G$ must correspond to a leaf in $G_{DS}$.
 TODO: probably rewrite, don't think I'm explaining it very well.
 
 Observe that if $u$ is an ancestor  of $v$ in $G$, then by the definition of consistency there must be a directed $s(u) - s(v)$ path in $N$.
 
 We begin with a technical claim that imposes some basic limitations on the structure of $G$ and $s$.
 
 \begin{claim}
  Let $rootSpec$ be the root of the subtree in $G$ corresponding to $spec_1$,
  and let $v$ be any leaf of the form $leafGeneEdge_j$ for $j \in [m]$, or $leafGeneIn_h$ or $leafGeneOut_h$ for $h \in [k]$.
  Then  any $s(rootSpec) - s(v)$ path uses at least one transfer arc.
  Furthermore such a path must pass through $tailVert_iIn$ for some $i \in [n]$.
 \end{claim}
\begin{proof}
 Since $s$ is a gene-species mapping, we have that $s(leafGeneEdge_j) = leafEdge_j$ for each $j \in [m]$ and $s(leafGeneIn_h) = leafIn$, $s(leafGeneOut_h) = leafOut$ for each $h \in [k]$.
 Observe that by construction of $N$, the only directed paths leading to $leafEdge_j$, $leafIn$ or $leafOut$ that do not use transfer arcs are those beginning with either $r$ or  some descendant of $y_0$.
 Therefore,to  prove the first claim,it will be enough to show that $s(rootSpec)$ is not $r$ and is not a descendant of $y_0$.
 
 Consider the root $spec_0$ of  $G_{DS}$ (and also of $G$). 
 As $spec_0$ is an ancestor of $leafGeneLeft$ and $leafGeneRight$, we must have that $s(spec_0) = r$, as this is the only node that is an ancestor of $leafLeft = s(leafGeneLeft)$ and $leafRight = s(leafGeneRight)$ in $N$.
 Furthermore, $spec_0$ cannot have been relabelled as a transfer node in $G$, as $r$ is not the tail of a transfer arc.
 Therefore $spec_0$ remains a speciation node in $G$.
 As $dup_0$ and $leafGeneRight$ are the children of $spec_0$, by definition of consistency the $r - s(dup_0)$ and $r - leafRight$ paths separate in $N$. 
 The $r-leafRight$ path necessarily has $y_0$ as its first node after $r$. 
 Therefore the $r - dup_0$ path cannot have $y_0$, and intead must have $x_0$ as its first node after $r$.
 Therefore $s(dup_0)$ is a descendant of $x_0$, from which it follow that $s(rootSpec)$ is a descendant of $x_0$ (as $rootSpec$ is a descendant of $dup_0$ in 
 $G$).
 As $s(rootSpec)$ is a descendant of $x_0$, it cannot be $r$ nor a descendant of $y_0$.
 
 (We note  that $N$ does  in fact have nodes that are descendants of both $x_0$ and $y_0$. However, all such nodes are descendants of the head of some transfer arc. Observe that no such node is an ancestor of  both $leafIn = s(leafGeneIn_1)$ and $leafEdge_1 = s(leafGeneEdge_1)$, which $s(rootSpec)$ is required to be.)
 
 So we now have that any $s(rootSpec) - s(v)$ path in $N$ uses at least one transfer arc.
 To see the second claim, observe that the every tail of a transfer arc in $N$ is a descendant of $tailVert_iIn$ for some $i \in [n]$. 
 (Every tail node was inserted between some $leafVert_i$  and its parent, and $tailVert_iIn$ was the first node added in this way.)
 \qed
\end{proof}
 
 
 Our next two claims show that for every $h \in [k]$, $s(dup_h)$ corresponds to a choice of vertex for our independent set $V'$.
 
 \begin{claim}
  For each $h \in [k]$, $s(dup_h)$ is an ancestor of $tailVert_iIn$ for some $i \in [n]$.
 \end{claim}
 \begin{proof}
 As $dup_h$ is  on the path from $rootSpec$ to $leafGeneIn_h$ in $G$, by the previous claim $s(dup_h)$ is either an ancestor or a descendant of $tailVert_iIn$ for some $i \in [n]$. 
 Note however that $tailVert_iIn$ itself is the only descendant of $tailVert_iEdge_j$ from which there are directed paths to both $leafIn = s(leafGeneIn_h)$ and $leafOut = s(leafGeneOut_h)$.
 As $dup_h$ is an ancestor of $leafGeneIn_h$ and $leafGeneOut_h$, this implies that $s(dup_h)$ is an ancestor of $tailVert_iIn$, as required.
 \qed
 \end{proof}
 
 From this point onwards, for each $h \in [k]$, let $i(h)$ be an arbitrary index such that $s(dup_h)$ is an ancestor  of $tailVert_{i(h)}In$.
 
 \begin{claim}
  For any $h,h' \in [k]$ such that $h \neq h'$, we have $i(h) \neq i(h')$.
 \end{claim}
 \begin{proof}
  Let $x = \lca_G(dup_h, dup_{h'})$, and note that $x$ is part of the subtree of $G$ corresponding to $spec_0$. As $spec_0$ was a speciation node in $G_{DS}$, $x$ is either a speciation node or a transfer node. As $dup_h$ is an ancestor of $tailVert_{i(h)}In$, and there is no ancestor of $tailVert_{i(h)}In$ that is the  tail of a transfer arc, (except for $tailVert_{i(h)}In$ itself), $s(x)$ cannot be the tail of a transfer arc. Therefore $x$ cannot be a transfer node, and so $x$ is a speciation node.
  (The case that $s(x)=s(dup_h)=s(dup_{h'}) = tailVert_{i(h)}In$ cannot occur, as in this case neither of the children of $s(x)$ take the transfer arc $(tailVert_{i(h)}In, headVert_{i(h)}In)$.)
  
  By the definition of consistency, the $s(x)-s(dup_h)$ and $s(x)-s(dup_{h'})$ paths must separate in $N$. 
  It follows that the descendants $tailVert_{i(h)}In$ of $s(dup_h)$ and $tailVert_{i(h')}In$ of $s(dup_h')$ must be distinct, and so $i(h) \neq i(h')$.
  \qed
 \end{proof}

 Thus, the set $V'= \{v_{i(1)}, \dots, v_{i(k)}\}$ is q set of $k$ vertices. 
 The next claim will allow us to  show that $V'$ is an independent set.
 
 For each $j \in [m]$ let $i[j]$ be an arbitrary index such that  $tailVert_{i[j]}In$ is on a  $s(rootSpec) - s(leafGeneEdge_j)$ path in $N$ (which must exist by the first claim).
 
 \begin{claim}
  For any $j \in [m]$ and any $h \in [k]$, we have $i[j]\neq i(h)$.
 \end{claim}
 \begin{proof}
 The proof is similar to the previous claim. 
 Let $x = \lca_G(leafGeneEdge_j, dup_h)$, and note that $x$ is part of the subtree of $G$ corresponding to $spec_0$.
 As $spec_0$ was a speciation node in $G_{DS}$, $x$ is either a speciation node or a transfer node.
 But as $dup_h$ is an ancestor of $tailVert_{i(h)}In$, and there is no ancestor of $tailVert_{i(h)}In$ that is the  tail of a transfer arc, (except for $tailVert_{i(h)}In$ itself), the only possibility for $x$ to be a transfer node is if $s(x)=s(dup_h)=tailVert_{i(h)}In$.
 But in this case neither the $s(x)_s(dup_h)$ path nor the $s(x)-s(leafGeneEdge_j)$ path in $N$ use the transfer arc $(tailVert_{i(h)}In, heqdVert_{i(h)}In)$, so this is impossible.
 
 Hence $x$ is a speciation node in $G$. 
 By definition of consistency,  the $s(x)-s(dup_h)$ and $s(x)-s(leafGeneEdge_j)$ paths must separate in $N$.
 It follows that the $s(x)-s(leafGeneEdge_j)$ path, and hence the $s(rootSpec) - s(leafGeneEdge_j)$ path, cannot pass through $tailVert_{i(h)}In$, and hence $i[j] \neq i(j)$.
 \qed
 \end{proof}
 
 
 We are now ready to put the proof together.
 
 Let $V'= \{v_{i(1)}, \dots, v_{i(k)}\}$. As
 we have $i(h) \neq i(h')$ for any  $h,h' \in [k]$ such that $h \neq h'$, .
 we have that $V'$ is a set of $k$ vertices. 
 To see that $V'$ is an independent set, observe that by the previous claim, for each edge $e_j$ the vertex $v_{i[j]}$ is not in $V'$.
 By definition $tailVert_{i[j]}In$ is on a  $s(rootSpec) - s(leafGeneEdge_j)$ path in $N$,
 and by construction of $N$, this can only happen if
 $N$ has the transfer arc $(tailVert_{i[j]}Edge_j, headVert_{i[j]}Edge_j)$, i.e.
 $v_{i[j]}$ is incident to $e_j$.
 Therefore every edge is incident with at least one vertex not in $V'$, from which it follow that $V'$ is an independent set.
 
\end{proof}




\begin{lemma}
 Suppose that $H$ has an independent set $V'$ of size $k$. Then there is a $CDST$-completion $G$ of $G_{DS}$ such that $G$ is consistent with $N$. 
\end{lemma}
\begin{proof}

Let $i_(1), \dots, i(h)$ be the set of indices such that $v_{i(1)}, \dots, v_{i(k)}$ are the vertices of $V'$.
For each $j \in [m]$, let $i[j]$ be an index such that $v_{i[j]}$ is a vertex incident to edge $e_j$ and not contained in $V'$. 
Note that such an $i[j]$ must exist, as $V'$ is an independent set.


We note now, as it will be relevant later, that for each $h \in [k]$ the node $tailVert_{i(h)}In$ is not an ancestor of $tailVert_{i[j]}Edge_j$ for any $j \in [m]$, nor of $tailVert_{i(h')}In$ for any $h' \neq h \in [k]$.


We now describe how to derive $G$ from $G_{DS}$, starting from the root and working down, describing the consistent gene-mapping $s$ as we go.
Note that intially $G$ will contain some unary speciation and transfer nodes. This will be fixed at the end of the construction.

Let $spec_0$ remain a speciation node and set $s(spec_0) = r$.
Let $s(leafGeneRight) = leafRight$
Let $dup_0$ remain q duplication node and set $s(dup_0)=x_0$.
Let $s(leafGeneLeft) = leafLeft$.

We will expand $spec_1$ into a binary subtree, with some of the nodes relabelled as transfer nodes.
The structure of the binary tree depends on our choices of $i(h), i[j]$ for $h  \in [k], j \in [m])$, and is constructed as follows.
Let $S'$ be the minimal subtree in $N$ that spans $tailVert_{i(h)}In$ for each $h \in [k]$ and  $tailVert_{i[j]}Edge_j$ for each $j \in [m]$.
Note that as $tailVert_{i(h)}In$ is not an ancestor of $tailVert_{i[j]}Edge_j$ for any $j \in [m]$, the node $tailVert_{i(h)}In$ is a leaf in $S'$ for each $h \in [m]$.
So let $S$ be the tree derived from $S'$ by removing the leaves  $tailVert_{i(h)}In$ for each $h \in [m]$.

We now expand $spec_1$ into a tree $T$ isomorphic to $S$. More specifically, $|V(T)| = |V(S)|$, and $s$ restricted to $V(T)$ is a one-to-one function such that for each $u,v \in V(T)$, $u$ is a child of $v$ if and only if $s(u)$ is a child of $s(v)$.
If $s(u) = tailVert_{i[j]}Edge_j$ for any $j \in [m]$, let $u$ be relabelled as a transfer node, and otherwise let $u$ remain a speciation node.

We next describe how the children of $spec_0$ in $G_{DS}$ are joined up to $T$ in $G$.
For each $j\in [m]$, let $s(leafGeneEdge_j) = leafEdge_j$, and let the parent of $leafGeneEdge_j$ be the transfer node $u$ for which $s(u) = tailVert_{i[j]}Edge_j$ .
(Note that the $tailVert_{i[j]}Edge_j - leafEdge_j$ path in $N$ uses the transfer arc $(tailVert_{i[j]}Edge_j ,headVert_{i[j]}Edge_j)$, satisfying the requirements of $u$ as a transfer node.)
For each $h \in [k]$, let $s(dup_h) = tailVert_{i(h)}In$, and let the parent of $dup_h$ be the $u$ such that $s(u)$ was the parent of $tailVert_{i(h)}In$ in $S'$.

Finally, for each $h \in[h]$, let $dup_h$ be relabelled as a transfer node, let $s(leafGeneIn_h) = leafIn$ and $s(leafGeneOut_h) = leafOut$.
Observe that this satisfies the requirement of $dup_h$ as a transfer node, since the $tailVert_{i(h)}In - leafIn$ path in $N$ uses the transfer arc $(tailVert_{i(h)}In , headVert_{i(h)}In)$.

Now contract any unary nodes to get the $CDST$-completion $G$ of $G_{DS}$.

Now we show that $s$ is  a consistent gene-species mappingfor $G$.
It is clear from the construction of $G$ and $s$ that $s$ is a gene-species mapping, and that for every node $u$ with child $v$ in $G$, there is a $s(iu)-s(v)$ path in $N$.
The only nodes of $G$ assigned to a tail of an arc in $E_s$ were those relabelled as transfer nodes, and we noted during the consturction of $G$ and $s$ that for each of these nodes $u$, the $s(u)-s(v)$ path took the corresponding transfer arc for one of $u$'s children $v$.

It remains to show that for each speciation node $u$ with children $v$ and $v'$, the $s(u) - s(v)$ and $s(u) - s(v')$ paths separate in $N$.
For speciation node $spec_0$, this is clear by inspection....
Every other speciation node is a node in $T$, the subtree of $G$ corresponding to $spec_1$.
Observe that as $s^{-1}(tailVert_{i[j]}Edge_j)$ and  $s{-1}(tailVert_{i(h)}In)$ were relabelled as transfer nodes for every $h  \in [k], j \in [m]$, for every speciation node $u$ in $T$ the node $s(u)$ is an internal node of $S'$. 
It follows by construction that if $u$ has distinct children $v$ and $v'$, then $(u)$ has distinct children $s(u)$ and $s(u')$. [NOTE TODO: actually this may not be true after contracting unary nodes, but the paths still separate.]
It follow that the $s(u) - s(v)$ and $s(u) - s(v')$ paths separate in $N$.


Thus, we have that $s$ is a consistent gene-species mapping for $G$, as required.
\end{proof}

%  In order to prove the claim, we will need to describe the $CDST$-completion $G$ and also a consistent gene-species mapping  $s:V(G) \rightarrow V(N)$.
% 
%  We will construct $G$ and $s$ concurrently, and afterwards show that $G$ is a $CDST$-completion of $G_{DS}$ and that $s$ is a consistent gene-species mapping.
% 
% 
%  
%  
%  Let $S$ be the subtree of $T_0(N)$ that spans $\{tailVert_{i(h)}In: h \in [k]\} \cup \{tailVert_{i[j]}Edge_j: j \in [m] \}$.
%  Note that for some $j \in [m]$, $tailVert_{i[j]}Edge_j$ will not necessarily be a leaf in $S$, as it may have a descendant $tailVert_{i[j']}Edge_{j'}$ (if $v_{i[j]}$ and $v_{i[j']}$ are the same vertex).
%  However, $tailVert_{i(h)}In$ will always be a leaf in $N$ for each $h \in [k]$, as $v_{i(h)} \neq v_{i[j]}$ for any $j \in [m]$.
%  
%  Now define a partial DST-tree $G'$ as follows.
%  
%  For 
%  
%  
%  
%  So let $S'$ be the tree dervied from $S$ be deleting the leaves $\{tailVert_{i(h)}In: h \in [k]\}$...
% [ Now describe how you take this tree and turn it into a subtree of $G$ corresponding to $spec_0$...]
%  We will now define the partof $G$ corresponding to $spec_0$... 
%  
%  For each.. hmmm
%  For each $v$ in $S$, let $s^{-1}(v)$ be a node in $G$, and let $s^{-1}(v)$ be a child of $s^{-1}(u)$ if and only if $v$ is a child of $u$.
%  All the nodes here are speciation nodes... but it's ok, by construction the thing holds....
%  Note that $S'$ is clearly a binary tree as it's a subtree of $T_0(N)$, which is binary.
%  
%  
%  
%  
% 
% 
% We first construct the $DST$-tree $G$, and then show that it is a a $CDST$-completion of $G_{DS}$ and consistent with $N$.
% 
% [Note: I'm bulding $G$ out of nodes in $G_{DS}$. I hope this is ok??]
% 
% 
% For each $j \in [m)$, let $leafGeneEdge_j$ be a leaf in $G$ with a new transfer node $geneTailVert_{i[j]}Edge_j$ as its parent.
% Let $s(leafGeneEdge_j) = leafEdge_j$, and $s(geneTailVert_{i[j]}Edge_j) = tailVert_{i[j]}Edge_j$.
% Observe that $tailVert_{i[j]}Edge_j, headVert_{i[j]}Edge_j, \dots, leafEdge_j$ is a path in $N$ from $s(geneTailVert_{i[j]}Edge_j)$ to $s(leafGeneEdge_j)$.
% 
% 
% 
% For each $h \in [k]$, let $leafGeneIn_h$ and $leafGeneOut_h$ be leaves in $G$, with  $dup_h$ as their parent.
% Let  $s(dup_h) = tailVert_{i(h)}In$.
% In addition let $s(leafGeneIn_h)= leafIn$, and  $s(leafGeneOut_h) = leafOut$.
% Observe that $tailVert_{i(h)}In, headVert_{i(h)}In, \dots, leafIn$ is a $s(dup_h)-s(leafGeneIn_h)$ path in $N$,
% and $tailVert_{i(h)}In, \dots, tailVert_iOut, headVert_iOut, \dots, leafOut$ is a $s(dup_h)-s(leafGeneOut_h)$ path in $N$.
% 
% 
% Now observe that...
% 
% 
% 
% Ok wait I have yet another way..
% 
% 
% Consider the minimal subtree in $N$ that spans $tailVert_{i[j]}Edge_j$ for each $j \in [m]$ and $tailVert_{i(h)}In$ for each $h \in [k]$.
% 
% HMMMM
% 
% 
% 
% 
% 
% % It will be convenient to partially define the values of $s$ (on nodes of $G$ that are also nodes of $G_{DS}$) before defining $G_{DS}$.
% 
%  First the leaf nodes: we assign $s(leafGeneRight) = leafRight, s(leafGeneLeft) = leafLeft$,
%  $s(leafGeneEdge_j) = leafEdge_j$ for all $j \in [m]$, and $s(leafGeneIn_h) = leafIn, s(leafGeneOut_h)=leafOut$ for  all $h \in [k]$.
%  We note at this point that for each leaf node $leaf$, $s(leaf)$ is equal to (the leaf node assigned to) the species assigned to (the gene assigned to) $leaf$, and so $s$ is a gene-species mapping.
% 
% %  Next, we assign $s(spec_0) = r, s(dup_0) = x_0, s(spec_1)=x_1$. 
% %  It remains to make assignments for $tailGeneEdge_j$ for each $j \in [m]$, and $dup_h, tailGeneOut_h$ for each $h \in  [k]$.
%  
% %  Let $i_1, \dots, i_k$ be the indices such that $v_{i_1}, \dots, v_{i_k}$ are the $k$ vertices in $V'$.
% %  Then for each $h \in [k]$, assign $s(dup_h) = tailVert_{i_h}In$ (recall that $dup_h$ was relabelled to be a transfer node), and assign $s(tailGeneOut_h) = tailVert_{i_h}Out$.
% %  For each $j \in [m]$, let $i_j$ be an arbitrarily selected index such that $v_{i_j}$ is incident with $e_j$ and $v_{i_j} \notin V'$. Note that such a $v_{i_j}$ must exist as $V'$ is an independent set. Now assign $s(tailGeneEdge_j) = tailVert_{i_j}Edge_j$ (noting that $tailVert_{i_j}Edge_j$ exists because $v_{i_j}$ is incident with $e_j$.
%  
%  Next, we assign $s(spec_0) = r, s(dup_0) = x_0$.
%  
%  
% 
%  We begin by describing how to derive $G$ from $G_{DS}$, which will be the same regardless of $V'$.
%  
%  We make the following subdivisions and relabellings.
%  For each $j \in [m]$, subdivide the arc between $leafGeneEdge_j$ and $spec_1$ with a new node $tailGeneEdge_j$. Label $tailGeneEdge_j$ as a transfer node ($TransSpec$ or $TransDup$, it doesn't matter), with $(tailGeneEdge_j, leafGeneEdge_j)$ a transfer arc.
%  
%  For each $h \in [k]$, relabel $dup_h$ as a transfer node (again, either $TransSpec$ or $TransDup$), and let $(dup_h, leafGeneIn_h)$ be the transfer arc.
%  In addition, subdivide the arc between $dup_h$ and $leafGeneOut_h$ with a new node $tailGeneOut_h$. Label $tailGeneOut_h$ as a transfer node; with $(tailGeneOut_h, leafGeneOut_h)$ a transfer arc.
%  
%  
%  We now give a consistent gene-species mapping $s:V(G) \rightarrow V(N)$.
%  
%  First the leaf nodes: we assign $s(leafGeneRight) = leafRight, s(leafGeneLeft) = leafLeft$,
%  $s(leafGeneEdge_j) = leafEdge_j$ for all $j \in [m]$, and $s(leafGeneIn_h) = leafIn, s(leafGeneOut_h)=leafOut$ for  all $h \in [k]$.
%  We note at this point that for each leaf node $leaf$, $s(leaf)$ is equal to (the leaf node assigned to) the species assigned to (the gene assigned to) $leaf$, and so $s$ is a gene-species mapping.
%  
%  Next, we assign $s(spec_0) = r, s(dup_0) = x_0, s(spec_1)=x_1$. 
%  It remains to make assignments for $tailGeneEdge_j$ for each $j \in [m]$, and $dup_h, tailGeneOut_h$ for each $h \in  [k]$.
%  
%  Let $i_1, \dots, i_k$ be the indices such that $v_{i_1}, \dots, v_{i_k}$ are the $k$ vertices in $V'$.
%  Then for each $h \in [k]$, assign $s(dup_h) = tailVert_{i_h}In$ (recall that $dup_h$ was relabelled to be a transfer node), and assign $s(tailGeneOut_h) = tailVert_{i_h}Out$.
%  For each $j \in [m]$, let $i_j$ be an arbitrarily selected index such that $v_{i_j}$ is incident with $e_j$ and $v_{i_j} \notin V'$. Note that such a $v_{i_j}$ must exist as $V'$ is an independent set. Now assign $s(tailGeneEdge_j) = tailVert_{i_j}Edge_j$ (noting that $tailVert_{i_j}Edge_j$ exists because $v_{i_j}$ is incident with $e_j$.
%  
%  This concludes the description of the gene-species mapping $s:V(G) \rightarrow V(N)$. It remains to show that $s$ is consistent.
%  
%  We first note that for every arc $(g, g_1)$ in $G$, there is a directed $s(g) - s(g_1)$ path in $N$, which is enough to satisfy the first condition of consistency.
%  In particular, 
%  For each $h \in [h]$, for the arc $(tailGeneOut_h, leafGeneOut_h)$ there is the path $s(tailGeneOut_h) = tailVert_{i_h}Out, headVert_{i_h}Out, \dots, leafOut = s(leafGeneOut_h)$.
%  For the arc $(spec_1, dup_h)$ there is the path $s(spec_1) = x_1, \dots, x_{i_h}, tailVert_{i_h}In = s(dup_h)$.
%  For each $j \in [m]$, for the arc $(spec_1, tailGeneEdge_j)$ there is the path $s(spec_1) = x_1, \dots, x_{i_j}, tailVert_{i_j}In, \dots, tailVert_{i_j}Edge_j = s(tailGeneEdge_j)$. TODO: VERIFY VERY CAREFULLY.
%  TODO: ANY OTHER COMPLICATED PATHS THAT NEED EXPLAINING?
%  
%  To satisfy the second condition of consistency, we first note that by construction, for any duplication or speciation node $g$, $s(g)$ is not the tail of an arc in $E_s$ (recall that $dup_h$ was relabelled to be a transfer node for each $h \in [k]$.
%  NOW PROVE THE SEPQRQTION THING IF THE FIRST VX IS A SPEC NODE G HAS CHILDREN G1 g2, DO THE PATHS IN SPEC NETWORK SEPARATE
%  
% \end{proof}  
%  
% A mapping $s : V(G) \rightarrow V(S)$ is called a \emph{gene-species mapping} if it
% satisfies $s(\l) = \sigma(\l)$ for each leaf $\l \in L(G)$.
% A gene-species mapping $s$ may possibly not be consistent with $T_0(N)$, nor with $N$ in the presence of transfers.
% Let $P_1 = x_0 x_1 \ldots x_{k}$ and $P_2 = x_0 x_1' \ldots x_{k'}$ be two directed paths starting at vertex
% $x_0$.  We say that $P_1$ and $P_2$ \emph{separate} if both paths have at least $2$ vertices and $x_1 \neq x_1'$.
% A \emph{consistent} gene-species mapping must satisfy the following properties 
% for each internal node $g$ with children $g_1$ and $g_2$:
% 
% \begin{itemize}
% 
% \item
% there exist a directed $s(g) - s(g_1)$ path $P_1$ and a directed 
% $s(g) - s(g_2)$ path $P_2$ in 
% $N$;
% 
% \item
%  
% if $g$ is a speciation or a duplication node, then $s(g)$ is not the tail of 
% an arc in $E_s$.  Moreover 
% if $g$ is a speciation node, then $P_1$ and $P_2$ separate;
% 
% \item
% if $g$ is a transfer node, then $s(g)$ is the tail of an arc $e$ in $E_s$, 
% and at least one of $P_1$ or $P_2$ takes the $e$ arc.
% 
% \end{itemize}
% 
% 
% TODO 
%   Note to self: does the current definition of consistent gene-species mapping have a nice place for duplication nodes to live? I guess they'd just go to the fist node in the species tree their descendants would pass through?



==> marksStuff.tex <==
% \section{DS-Trees with gene transfer}


Given a rooted tree $T$, let $L(T)$ denote the leaves (labels on leaves?) of $T$.
The root of $T$ is denoted $r(T)$, 
and the subtree rooted at node $x$ is denoted $T_x$.
Let $I(T)$ denote the internal nodes of $T$.
Given two nodes $x,y$ in $T$, let $\lca_T(x,y)$ denote the least common ancestor of $x$ and $y$ in $T$.
We call $x$ and $y$ \emph{separated} if $\lca_T(x, y) \notin \{x, y\}$.


\subsection{DST-trees}

Let $V$ be a set of genes. %, and $s: V \rightarrow \Sigma$ a species assignment mapping genes to species.
 A \emph{DST-tree for $V$} is a pair $(T,l)$, where $T$ is a rooted tree with set $L(T) = V$, and
  $l:I(T) \rightarrow  \{Dup, Spec, TransSpec, TransDup \}$ is a function labelling each internal node of $T$ as a \emph{duplication, speciation} or \emph{transfer} node, which can be interpreted as either a speciation or a duplication (biological meaningfulness?).
 In addition we assume that a transfer node is binary, and one of its two out-arcs is a \emph{transfer arc}. 
 (The transfer node/arc represents a gene being transferred from one species to another - if $z$ is a transfer node with children $x,y$ and $(z,y)$ is the transfer arc, then a copy of $z$ was transferred into another species and became $y$.)
We will write $T$ to denote the DST-tree $(T,l)$ when $l$ is clear from context.
 [NOTE: WHAT ABOUT TRANSFER-LOSS NODES?  I don't want to mess this up.  I will try my own defs in my section.]
 
 
 Given $x,y \in V$, we say that $x$ and $y$ are \emph{orthologs} w.r.t $T$ if $\lca_T(x,y)$ is a speciation 
 or a transfer-speciation node. %{\bf or a transfer node}.
 We say $x,y$ are \emph{paralogs} w.r.t $T$ if $\lca_T(x,y)$ is a duplication or a transfer-duplication node.
In addition, we say that $x$ and $y$ are \emph{xeno}-orthologs or \emph{xeno}-paralogs (?) if the undirected path between $x$ and $y$ in $T$ contains a transfer arc (NOTE ML: I'm not sure it's necessary).
Note that unary nodes can never be the $lca$ of two leaves.

Given a DST-tree $(T,l)$ for $V$, we say a graph $G=(V,E)$ is the \emph{relation graph of $T$} (or that $T$ is a \emph{DST-tree for $G$}) if the following holds:
The edge $xy \in E$ if and only if $x,y$ are orthologs w.r.t $T$ (that is, $\lca_T(x,y)$ is a speciation or transfer-speciation node).  In this case we say that $T$ \emph{displays} $G$.


\subsection{Species trees and LGTs}


Let $s: V \rightarrow \Sigma$ denote a \emph{species assignment} mapping genes to species.

A \emph{species tree on $\Sigma$} is a rooted tree with $L(S)=\Sigma$.

\medskip
We now attempt to define an  \emph{LGT(lateral gene transfer) on $\Sigma$}. [This definition probably needs some work.]

Let $H=(X,A\uplus B)$ be an acyclic directed graph, where $X$ are the nodes of $H$ and $A\uplus B$ are the arcs of $H$.
We call $A$ the \emph{normal arcs}(???) and $B$ the \emph{transfer arcs} of $H$.

Let $H'$ denote the directed graph derived from $H$ by deleting all transfer arcs, and contracting all vertices of in-degree and out-degree $1$. (These should be the nodes that were previously adjacent to transfer arcs).

Then we say that $H$ is an \emph{LGT for $\Sigma$} if 
\begin{itemize}
 \item $H'$ is a species tree on $\Sigma$ (i.e. $H'$ is a tree and $L(H')=\Sigma$).
 \item If $xy$ is a tranfer arc, there is be no directed path from $x$ to $y$ in $H$ that does not use the arc $xy$ (in particular, this means that you canot transfer genes from an ancestral species to its descendant, and that transfer arcs should not be able to 'cross' each other)
 \item Other properties???? 
\end{itemize}



\subsection{Consistency}

QUESTION: How do we define consistency of a DST-tree with an LGT?

Intuitively, it should be that the DST-tree can be ``embedded'' within the LGT.

What about consistency of a DST-tree with a species tree?

% Attempt:
% Given a DST-tree $T$ on $V$, a species assignment $s:V \rightarrow \Sigma$, and an LGT $H$ on $\Sigma$, we say that \emph{$T$ is consistent with $H$} if the following holds:
% 
% \begin{itemize}
%  \item 
% \end{itemize}



\subsection{Problems to look at}



\begin{definition}[Consistency with LGT]
\\
{\bf Input}: A graph $G = (V,E)$, a species assignment $s:V \rightarrow \Sigma$, and an LGT $H$ on $\Sigma$.\\
{\bf Question}: Does there exist a DST-tree $T$ for $G$ such that $T$ is consistent with $H$? 
\end{definition}

\begin{definition}[Transfer Optimization with LGT]
\\
{\bf Input}: A graph $G = (V,E)$, a species assignment $s:V \rightarrow \Sigma$, and an LGT $H$ on $\Sigma$.\\
{\bf Question}: Find a DST-tree $T$ for $G$ such that $T$ is consistent with $H$ and the number of transfer nodes in $T$ is minimized. 
\end{definition}

We can also consider:
\begin{itemize}
 \item The variation where we are not given an LGT but just a species tree $S$, and we may have transfer arcs anywhere.
 \item The variation where are not given an LGT  or a species tree and need to find a species tree for ourselves.
 \item The variations where we have some unknown edges that could be orthologs or paralogs.
 \item And probably some others...
\end{itemize}


==> satOOCReduction.tex <==

Here we sketch a NP-hardness proof for deciding whether a set of relations $R$ can be displayed
by a $CDST$-tree, even if $S(H)$ is time-consistent.
We use a reduction from the \satpb problem, which consists in deciding whether a boolean formula in CNF form 
is satisfiable, with the additional constraints that each clause has $2$ or $3$ variables, 
and each variable appears in $2$ or $3$ clauses (counting every positive or negative appearance).
[REF: Tovey, 1984]
We may assume that each variable $x_i$ appears positively and negatively at least one time.

Let $\phi$ be a \satpb instance, with variables $\{x_1, \ldots, x_n\}$ 
and clauses $\C = \{ C_1, \ldots, C_m \}$.  The ordering of the $x_i$'s can be arbitrary, 
but must remain fixed as it will be of importance later on.
From $\phi$ we construct a corresponding instance of $RET$, that is a relation graph $R$, a species tree $S$ 
and transfer highways $H$.

We start by constructing $S$ and $H$.  As an intuitive aid, the whole point of this construction is to build a species network
that allows, for some specific gene trees $G_1, \ldots, G_m$ which we describe later, multiple choices
for each $s(r(G_i))$ by allowing transfers.  We will construct the trees so that $\phi$ is satisfiable 
iff $s(r(G_1)), \ldots, s(r(G_m))$ can be chosen to be pairwise-separated in $S$ (and thus pairwise related by speciation) .


 
Let $x_i$ be a variable of $\phi$, and define a corresponding tree $X_i$
(of which the root is of degree one, as it will become a transfer node), in the following way:

\begin{itemize}


\item
if $x_i$ appears twice positively in clauses $C_{j_1}$ and $C_{j_2}$, and once negatively in clause $C_k$, 
then let $X_i'$ be a binary tree with $3$ leaves.  Insert a degree one node labeled $(x_i, C_k)$ by connecting it to 
$r(X_i')$ by an edge, and set it as the new root of $X_i'$.
Moreover take any $2$ leaves and label them by $(x_i, C_{j_1})$ and $(x_i, C_{j_2})$.  
Label the other leave $\l(x_i, C_k)$.
To obtain $X_i$, add $2$ new pending leaves: one leaf $\l(x_i, C_{j_1})$ connected to $(x_i, C_{j_1})$, 
one leaf $\l(x_i, C_{j_2})$ connected to $(x_i, C_{j_2})$.


\item
if $x_i$ appears once positively in clause $C_{k}$, and twice  negatively in clauses $C_{j_1}$
and $C_{j_2}$,  
apply the same construction as above.


\item
if $x_i$ appears only twice in $\C$, say positively in clause $C_j$ and negatively in clause $C_k$, 
then $X_i$ consists of a path of length $2$ (i.e. a $P_3$) with nodes $a, b, c$ and edges $ab$ and $bc$, 
to which we add two leaves adjacent to $c$ ($X_i$ is known as a \emph{fork}).    
Assign the $a$ node as the root, and label it $(x_i, C_j)$.  
Label the $b$ node by $(x_i, C_k)$, 
and label the inserted leaves $\l(x_i, C_j)$ and $\l(x_i, C_k)$.

\end{itemize}


Intuitively, to each variable $x_i$ and clause $C_j$ appearance corresponds a transfer node 
$(x_i, C_j)$ in $X_i$.  If some clauses $C_j$ and $C_k$ contain $x_i$ with the same value 
(i.e. both positive or both negative), then $(x_i, C_j)$ and $(x_i, C_k)$ are separated in $X_i$.
Otherwise, one of $(x_i, C_j)$ or $(x_i, C_k)$ is an ancestor of the other.  The pending leaves are added so that 
each $(x_i, C_j)$ node has its own corresponding leaf $\l(x_i, C_j)$ in $X_i$.
Call a node of $X$ \emph{marked} if it labeled by some $(x_i, C_j)$.

Let $X'$ be any tree containing each $X_i$ separately, i.e. take a tree on $n$ leaves, 
then replace each leaf by the root of a distinct $X_i$.
Obtain the tree $X$ by adding a new leaf $\alpha$ as an outgroup, that is 
by connecting $\alpha$ and $r(X')$ under a common parent.

To obtain $S$ we add transfer nodes to $X$, and construct the transfer highways $H$.
For each marked node $(x_i, C_j)$ in $X$, add a transfer node $\alpha_{ij}$ 
on the $\{r(X), \alpha\}$ edge, making sure that if $(x_i, C_j)$ has a marked descendant, 
$(x_{i}, C_{k})$, then $\alpha_{ij}$ lies above $\alpha_{ik}$ (i.e. $\alpha_{ij}$ is closer to the root).
Then, add to $H$ the transfer highway $( (x_i, C_j), \alpha_{ij})$ to $H$.
Thus from $(x_i, C_j)$, one can always transfer to $\alpha$.
It is not hard to see that time-consistency is preserved by the inserted transfer highways.
[NOTE: we should assign precise time slots]

We finally describe transfers between $X$ leaves, and in the meantime provide a time slot for each transfer node.
For each leaf $\l(x_i, C_j)$, let $e_{ij}$ be the edge between $\l(x_i, C_j)$ and its parent.
Add exactly $n - i + 1$ transfer nodes 
$t^{ij}_{i}, t^{ij}_{i + 1}, \ldots, t^{ij}_{n}$ on the $e_{ij}$ edge, and assign $t^{ij}_{k}$ the time slot $k$,
for each $i \leq k \leq n$.  This finishes the construction of $S$.
As for $H$, for each clause $C_j \in \C$ containing 
variables $x_{a}, x_{b}$ and $x_{c}$ with $a < b < c$, add to $H$ the transfer highways 
$(t^{bj}_{b}, t^{aj}_{b})$ and $(t^{cj}_{c}, t^{aj}_{c})$.
[NOTE: WTF is this construction?]
The point of these transfers is to allow a path from  
$(x_b, C_j)$ and $(x_c, C_j)$ to $\l(x_a, C_j)$.
Note that for some $i$, the highest (i.e. oldest) transfer node $t^{ij}_i$ is always 
the donor, whereas the lower ones are the receivers.  Moreover a donor $t^{ij}_i$ can only 
give to a receiver $t^{i'j}_i$ with $i' < i$.
[NOTE: intuitively, all transfers go 'to the left', which somehow enforces time consistency.
Formal details to come.]

We now construct a set of relations $R$, or more precisely a least resolved $DS$-tree $G$ for $R$
(they are in 1-to-1 correspondence).
For each  clause $C_j \in \C$ with variables $x_{a}, x_{b}, x_{c}$ with $a < b < c$, 
we first build a corresponding subtree $G_j$.
The tree $G_j$ is a binary tree on $2$ leaves, one of which is labeled $\alpha$, 
and the other $\l(x_a, C_j)$ (we label genes by their corresponding species).
The $DS$-tree $G$ is obtained by taking a polytomy on $m$ children $1, \ldots, m$, then replacing 
each child $j$ by $G_j$.
The root of $G$ is a speciation, whereas every other internal node (i.e. the $G_j$ roots) is a duplication.
By Lemma~\ref{lem:refinement}, $R$ can be displayed by a $CDST$-tree if and only if
$G$ admits a binary refinement for which there is a $CDST$-completion $G'$. 
We show that $G'$ exists if and only if $\phi$ is satisfiable.
The proof is divided in a series of claims.

\begin{claim}
For every $C_j \in \C$
with $C_j = (x_a \vee x_b \vee x_c)$ and $a < b < c$, by using transfers $s(r(G_j))$ can be any of $(x_a, C_j), (x_b, C_j)$ or $(x_c, C_j)$.  Moreover $s(r(G_j))$ must be an ancestor of one of those nodes.
\end{claim}

\begin{proof}
Denote $r = r(G_j)$.
To verify the first assertion, first notice that $s(r) = (x_a, C_j)$ is possible if 
$\{r, \alpha\}$ is made a transfer arc and $\{r, \l(x_a, C_j)\}$ a regular edge.
If instead $s(r) = (x_b, C_j)$, then make $r\alpha$ a transfer edge, 
add a transfer-loss node mapped to $t^{bj}_b$ on the other edge, and transfer to $\l(x_a, C_j)$. 
The case $s(r) = (x_b, C_j)$ is identical.

For the second assertion, suppose that $s(r)$ is not an ancestor of one of the specified nodes.
Observe that in this case, there is no directed path from $s(r)$ to $\l(x_a, C_j)$ in $S(H)$.
Thus the $\{r, \l(x_a, C_j)\}$ edge cannot be a transfer arc.  But then, $s(r)$ is not an ancestor of 
$\l(x_a, C_j)$, and so $s$ is not a valid gene-species mapping.
\qed
\end{proof}

\begin{claim}
Let $G'$ be a $CDST$-completion of a binary refinement of $G$.  Then the only transfer arcs of $G'$ 
have tail $r(G_j)$ for some $1 \leq j \leq m$.
\end{claim}

\begin{proof}
Suppose that in $G'$, there is a transfer arc $(x, y)$ on the path between the root and $r(G_j)$
for some $j$. Choose $(x, y)$ to be farthest from the root as possible.  By the previous claim, 
$s(r(G_j))$ must be an ancestor of $(x_i, C_j)$ for some $i$.  Since there is no transfer on the path between $y$ and $r(G_j)$, $s(y)$ must be an ancestor of $s(r(G_j))$.  But there is no transfer arc that leads
to $y$ nor any of its ancestors, and therefore the $(x, y)$ transfer arc is not feasible.
\qed
\end{proof}

\begin{claim}
$G$ admits a binary refinement for which there is a $CDST$-completion $G'$ 
if and only if there is a choice of $s_1 = s(r(G_1)), s_2 = s(r(G_2)), \ldots, s_m = s(r(G_m))$ 
such that $s_1, s_2, \ldots, s_m$ are pairwise-separated in $S$.
\end{claim}

(proof idea: every node above the $G_j$'s needs to be a speciation.)

\begin{claim}
There is a choice of $s_1 = s(r(G_1)), s_2 = s(r(G_2)), \ldots, s_m = s(r(G_m))$ 
such that $s_1, s_2, \ldots, s_m$ are pairwise-separated in $S$ if and only if $\phi$ is satisfiable.
\end{claim}

(proof idea: $(\Rightarrow)$ the 
choice of $s(r(G_j)) = (x_i, G_j)$ corresponds to setting $x_i$ to the value that satisfies the clause $C_j$.  No literal is chosen both true and false, by the $X_i$ construction.  
$(\Leftarrow)$ if $C_j$ is satisfied by $x_i$, set $s(r(G_j)) = (x_i, C_j)$.  Pairwise-separation follows since 
positive-negative pairs can't both be chosen.
 
 
